From Waterfallish Aerospace Certification onto Agile Certifiable Iterations

Agile software development is becoming increasingly popular in the aerospace industry because of its capability to accommodate requirement changes. However, safety-critical domains require compliance with strict regulations such as the DO-178C avionics standard, which demands thorough documentation. The main challenge of this constraint is not the content itself, but rather the comprehensive traceability from system-level requirements to all sorts of testing and verification evidence, including who did what, when, and to which artifact. Currently, this is mostly a manual activity performed at the end of the project, which blocks efforts to agilize the development of software for aerospace applications. In this paper, we present a strategy and tools that support the generation of continuous documentation complying with DO-178C requirements. By iteratively creating the DO-178C documentation associated with each software component and seamlessly merging it with the previously generated documentation, we open the way to truly continuous certifiable iterations, an evolution from the current Waterfallish industry practice. The proposed mechanisms and tools were co-designed and validated with aerospace industry professionals, thereby confirming its applicability and usefulness. The generated artifacts show that document automation is feasible in the aerospace industry, opening the way for more widespread adoption of Agile practices in this highly regulated sector.

==> 4-summary.tex <==
\subsection{Summary}
In summary, the aerospace software development process is highly complex and demanding due to the elevated level of compliance required from standards such as the \emph{DO-178C}. Also, as stated in~\cite{Ribeiro2023}, during the entire process, including documentation, great  effort is required for V\&V activities to ensure compliance with the DO-178C standard. The proposed automated solution streamlines documentation creation and management, targeting the most demanding artifacts , the SRD and the SCI, while enabling safety engineers to write requirements in their IDE. This solution connects existing tools like Jira, IBM DOORS, and Bitbucket, facilitating the automated generation of certifiable data packages. Finally, incremental packages containing essential artefacts are generated and validated before certification. This structured approach enhances documentation efficiency and supports compliance with regulatory standards for this research, specifically the \emph{DO-178C}, ultimately expediting the certification process.

